Modeling Student Performance in Game-Based Learning Environments

This study investigates game-based learning in the context of the educational game "Jo Wilder and the Capitol Case," focusing on predicting student performance using various machine learning models, including K-Nearest Neighbors (KNN), Multi-Layer Perceptron (MLP), and Random Forest. The research aims to identify the features most predictive of student performance and correct question answering. By leveraging gameplay data, we establish complete benchmarks for these models and explore the importance of applying proper data aggregation methods. By compressing all numeric data to min/max/mean/sum and categorical data to first, last, count, and nunique, we reduced the size of the original training data from 4.6 GB to 48 MB of preprocessed training data, maintaining high F1 scores and accuracy. Our findings suggest that proper preprocessing techniques can be vital in enhancing the performance of non-deep-learning-based models. The MLP model outperformed the current state-of-the-art French Touch model, achieving an F-1 score of 0.83 and an accuracy of 0.74, suggesting its suitability for this dataset. Future research should explore using larger datasets, other preprocessing techniques, more advanced deep learning techniques, and real-world applications to provide personalized learning recommendations to students based on their predicted performance. This paper contributes to the understanding of game-based learning and provides insights into optimizing educational game experiences for improved student outcomes and skill development.

==> tex/Instructions.tex <==
Report. Each team will submit a final project report. If you did this work in collaboration with someone else, or if someone else (such as another professor) had advised you on this work, your write-up must fully acknowledge their contributions.

Format: A PDF document that is between 6-12 pages (single columns and no smaller than 11-point font) with additional pages for references.  Suggested length (not required): 6-8 pages for 1 or 2 person teams, 10-12 pages for 3-4 person teams.  The typical ingredients of a project report are:

Abstract (abstract) (1-2 paragraphs) (ANTHONY)
Introduction: What is the problem being addressed? Why is it important? Overview and high-level rationale of your approach. Highlight the novelty, key contributions, or significance of your project.

Background (related-work) (ANTHONY)
: Past related work on the problem done by others.

Methods (approach) : (SUSANNA) (ADD PSEUDO-CODE ALGORITHM FUNCTION)
Describe your learning algorithms or proposed algorithm(s). Introduce any relevant mathematical notation if needed. For each algorithm, give a short description of how it works. For algorithms covered in class, this can be 1-3 sentences to convey why it might be useful for this problem. If you are using a niche or cutting-edge algorithm, you may want to explain your algorithm in 1-2 paragraphs.

Experiments/Results (experiments) (HARRY HE)
    Data description    (EXPLAIN ALL THE FEATURES) (NICE VISUALIZATION)
    Exploratory data analysis, preprocessing, feature extraction, feature selection: Enough to ensure your experiments can be replicated by others

    (HARRY BELOW)
    Modeling choices: What models did you select? Why? How were parameters determined? Other design choices such as subsampling, oversampling, etc.
    Empirical results and comparisons (figures and tables)
    
Discussion (analysis): 
What are the key findings and lessons learned from the experiment?

Contributions: Please include a section that describes what each team member worked on and contributed to the project. We may reach out and factor in contributions and evaluations when assigning project grades.





Code/dataset: Please include a link to either a Github repository, Google drive folder, or Dropbox folder with the code and dataset for your final project.  


==> tex_old/abstract.tex <==
\begin{abstract}

Game-based learning is a new educational technique that utilizes games as a method of learning. It has the potential to increase student engagement, decrease anxiety around learning, increase performance while also being widely accessible and having the ability to be tailored to each individual student. 
ADD MORE.



\end{abstract}

==> tex_old/acknowledgements.tex <==
\section*{Acknowledgements}

We thank Agustin Volante, Jacqueline Lin, Kevin Park, Matias Moreno, and Ryan Lin for their contributions to establishing the human performance benchmarks for ScholasticQA. We also thank Jinho Choi for his guidance, and gratefully acknowledge support from Kaustubh Dhole and Sichang Tu in developing the manuscript.

==> tex_old/analysis.tex <==
\section{Discussion}
\label{sec:analysis}






\subsection{Performance  Analysis}
\label{sec:panalysis}
\begin{table}[htbp!]
\centering\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cccc} 
\toprule
\bf Language Model & \bf Easy & \bf Medium & \bf Hard & \bf Overall \\
\midrule
BERT Base & 46.34 & 23.81 & 26.32 & 35.80 \\
BERT Large & 48.78 & 33.33 & 21.05 & 38.27 \\
DistilRoBERTa & 51.22 & 38.10 & 26.32 & 41.98 \\
RoBERTa Base & 56.10 & 38.10 & 31.58 & 45.68 \\
RoBERTa Large & 58.54 & 42.86 & 36.84 & 49.38 \\
\hline
Humans & 87.80 & 80.95 & 68.42 & 81.67 \\
\bottomrule
\end{tabular}}
\caption{Performance accuracy on GRE question dataset, with all question types (1-, 2-, or 3-blanks) classified by difficulty annotations rather than number of blanks. All models are off-the-shelf and have not been finetuned or further trained beyond the pretraining detailed in the original work \cite{devlin-jacob-2019-BERT, liu-etal-2019-roberta}.}
\label{tab:difanalysis}
\end{table}


Interestingly, model performance on questions classified as "hard" were significantly lower than that of questions classified as "easy", despite the fact that hard questions generally had longer text lengths due to the nature of GRE questions; most "hard" questions involved 2- and 3-blank questions (as opposed to 1-blanks questions), which meant that the overall length was typically longer to accommodate for more answer choices. This likely influences accuracy performance given that model performance directly depends on the amount of context given, which is important for masked language modeling tasks. Thus, acknowledging that these official GRE questions only represent a subset of our overall dataset, it is possible that performance on hard questions is more contingent on overall difficulty (e.g., grammatical concepts, sentence structure, overall comprehension) than text length. It is notable that this idea is further supported by our human performance data, which also showed a significant decrease in accuracy for "hard" questions compared to "easy" and "medium" questions.

\subsection{Error Analysis}
\label{sec:eanalysis}

Manual annotation of 60 randomly sampled errors from our experimental results in Tables \ref{tab:experimentresults} and \ref{tab:difanalysis} were performed to provide insights for future research directions. Table \ref{tab:erroranalysis} exhibits the three major types of errors revealed through our analysis:
\begin{itemize}
    \item \textbf{Close Match} This type of error occurs when the probability distribution of answer choices generated by the models used exhibit close values for two of the answer choices (out of 5 for 1-blank questions and 3 for 2- and 3-blank questions), which we define to be anything less than 5\%; the correct answer turns out to be the one that isn't chosen by the model, so it is categorized as a "close match" error. This signifies the difficulty for pretrained models to disambiguate between two answer choices given limited context, and overcoming this error type likely requires a more advanced attention mechanism to focus on specific spans (rather than processing the entire text), as discussed by \citet{berzak-yevgeni-2020-STARC}).
    \item \textbf{Relational Context} This type of error occurs in 2- or 3-blank questions, where subordinating conjunctions can often confuse the model in regards to choosing a "positive" or "negative" candidate; a sample question text completion question is as follows: "The gaps in existing accounts of the playwright's life are not \_\_\_, since much of the documentary evidence on which historians have relied is \_\_\_." In this case, the model must infer that the conjunction "since" implies that the second candidate chosen (in regards to the "evidence") must refer to and support the "gaps" mentioned in the first part of the sentence. These types of relational context errors extend beyond simple sentence structures, revealing a significant challenge in developing machine models with the ability to reason across complex relationships between different parts of a given sentence; it is likely that the RoBERTa models used in our experiments can do this better than the BERT models, thus reflecting the higher performance scores in Table \ref{tab:difanalysis}.
    \item \textbf{Miscellaneous} Errors labeled as miscellaneous have no identified cause for understanding why the models used in our experiments predict incorrect candidates, thus requiring further investigation into the underlying transformer architecture.
\end{itemize}

\begin{table}[htbp!]
\centering\resizebox{\columnwidth}{!}{
\begin{tabular}{cccc} 
\toprule
\bf Error Analysis & \bf Close Match & \bf Relational Context  & \bf Miscellaneous \\
\midrule
Distribution & 45\% & 21\% & 34\% \\
\bottomrule
\end{tabular}}
\caption{Error distributions across the three types analyzed in the 60 randomly sampled candidates from experimental results in Tables \ref{tab:experimentresults} and \ref{tab:difanalysis}.}
\label{tab:erroranalysis}
\end{table}
Given this performance and error analysis, it is our hope that the challenges described above can be tackled by future studies. To the best of our knowledge, this is the first paper to present findings on GRE-like text completion and sentence-equivalence questions, featuring multiple blanks as opposed to traditional single-blank questions \cite{zweig-burges-2012-challenge}; acknowledging that the dataset utilized here does not reach the sample size of larger, state-of-the-art reading comoprehension question banks such as RACE and OneStopQA \cite{lai-guokun-2016-RACE, berzak-yevgeni-2020-STARC}, a collective effort in producing similar standardized examination questions and comparing model performance on improved datasets will allow for better extrapolation and generalizability. Furthermore, the development of language models with attention mechanisms focused on specific spans (as described by \citet{berzak-yevgeni-2020-STARC}) may allow for the generation of better encodings, ultimately translating to higher accuracy scores due to the nature of these examination questions: they are fundamentally designed to test comprehension, rather than understanding of context-independent grammatical relationships.  





==> tex_old/approach.tex <==
\section{Approach/Method}
\label{sec:approach}

INCLUDE THE MATH NOTATION BEHIND IT
Methods (approach) : Describe your learning algorithms or proposed algorithm(s). Introduce any relevant mathematical notation if needed. For each algorithm, give a short description of how it works. For algorithms covered in class, this can be 1-3 sentences to convey why it might be useful for this problem. If you are using a niche or cutting-edge algorithm, you may want to explain your algorithm in 1-2 paragraphs.



In this section, we will present our approach to the initial data exploration in addition to the methods of our data pre-processing and the machine learning techniques that we used to classify the observations.




\subsection{Machine Learning Techniques}

We trained models K-Nearest Neighbors (KNN) with k = 5 and Multilayered Perceptron models on our data. 

KNN is a commonly used machine learning classifier that is useful because it does not make assumptions about the underlying distribution of the data. One of its main drawbacks is that it suffers from the curse of dimensionality where as the number of features increases, the amount of observation needed to obtain a good accuracy exponentially increases. In this case, this is not an issue as our dataset is large and there are not that many features that we kept from pre-processing. The drawback of KNN is that it is computationally expensive as the model needs to store all of the training data and calculate each distance. 

Multilayered Perceptron is a machine learning technique that uses multiple layers of perceptrons that are fully connected in an artificial neural network. In a single perceptron, inputs (features) are assigned weights. The weighted sum of the features will allow the classifier to predict if an observation is positive or negative based on its comparison to a threshold. The weights are adjusted iteratively to minimize 0-1 loss. With a single perceptron, the data must be linearly separable, but with multiple layers, this is not necessary. the weights and biases are updated by the model's performance on each data point. One of the drawbacks of neural networks is that the results are not interpretable and the model does not produce information about the correlations of the features to the label or the feature importance.

The third machine learning technique that we used is Random Forest. In Random Forest, multiple decision trees are modeled on the data in order to produce multiple predictions which are combined together in a majority vote to produce one prediction. In a decision tree, the data is partitioned using features and threshold values. 





TABLE WITH RESULT -> analysis section
STATE OF ART (COMPARISON) -> analysis or conclusion

for analysis
summarize briefly about the result. Mention about different preprocessing methods and how it can affect the result. Or how it affected "our" result. Also, mention about why one model performs better than others.

******DELETE BELOW TEXT:******
This section presents our data collection process, in addition to the deep learning neural architectures used for our text completion models; our approach features a variety of state-of-the-art language modeling methods, allowing for baseline statistics to be established for the dataset with BERT and RoBERTa \cite{liu-etal-2019-roberta, zhuang-etal-2021-robustly}. An advanced method with fine-tuning is also conceptually compared to expand beyond previous work and establish comparative statistics on accuracy for the dataset.

\subsection{Data Collection and Statistics}
\label{sec:data}

This paper presents a new text completion dataset based on collections of verbal reasoning and writing questions taken from GRE and SAT practice exams. Such problems are referred to as cloze questions (denoted as \( \mathit{Q} \)), where each question in the dataset consists of three parts: 
\begin{enumerate}
    \item A passage \( \mathit{P} \) composed of one to six sentences
    \item A series of one to three blanks \( \mathit{B} \) in \( \mathit{P} \), where each will correspond to a correct answer choice to be selected
    \item A set of candidates or answer choices \( \mathit{C} \) for each blank, where they are independent across different blanks (i.e., the answer choice for one blank does not affect the available choices for a separate blank)
\end{enumerate}

Cloze questions are crawled from public websites with substantial collections of SAT and GRE questions in order to maximize the scope and relevancy of the problems tested\footnote{https://gre.viplgw.cn/search.html?page=1; https://www.myuniuni.com/examination/sat/list?page=1}; in addition, following previously work on NLP tasks centered on machine reading comprehension and question answering for test examinations \cite{woods-2016-exploiting}, sentence completion questions were directly sourced from official sources such as the College Board and Educational Testing Service to allow for direct comparisons of baseline accuracy results\footnote{https://satsuite.collegeboard.org/sat/practice-preparation/practice-tests/paper; https://www.ets.org/gre/test-takers/general-test/prepare/powerprep.html}. However, it is worth noting that questions were also sourced from unofficial test preparation websites and databases, in order to increase the number of questions available for model training described in Section \ref{sec:methods} and introduce novel passages to expand beyond previous work. Automation scripts were built with Selenium to scrape the questions, and when they involved images that contained the answers (as opposed to the text themselves), an OCR engine\footnote{https://github.com/tesseract-ocr/tesseract} was utilized to transcribe them into the standard textual format described above with a set of answer choices \( \mathit{C} \) for each blank in the question. In total, 305 questions were collected from the databases and websites listed. Sample questions from our dataset are shown in Figure \ref{fig:sampleqs}. 

In order to adjust for inconsistencies and remove any faulty questions, the following steps were conducted to clean the raw dataset. First, any questions that had a missing component (either the passage \( \mathit{P} \), the existence of at least one blank \( \mathit{B} \), or the set of answer choices for each blank \( \mathit{C} \)) were discarded. Second, any duplicate questions were filtered out and removed. Lastly, for all \( \mathit{Q} \) such that \exists \; a \, \( \mathit{B} \) without a corresponding \( \mathit{C} \) (i.e., more blanks than answer choices), these questions were discarded as well.

After pre-processing the data with the steps above, our final dataset is complete with 305 questions. More granular and detailed statistics can be found in Table \ref{tab:dataset}. 

\begin{table}[htbp!]
\centering\small{ %\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c} 
\toprule
\bf Type & \bf Value \\
\midrule
Total questions & 305  \\
Total blanks & 519  \\
\# of 1-blank questions & 162 \\
\# of 2-blank questions & 98 \\
\# of 3-blank questions & 45 \\
Average passage length in words  & 25.4  \\
Average blanks per passage & 1.70 \\
\# of candidates for 1-blank questions & 5 \\
\# of candidates for 2- and 3-blank questions & 3 \\
\bottomrule
\end{tabular}}
\caption{Detailed statistics of the pre-processed dataset of sentence completion questions}
\label{tab:dataset}
\end{table}

\begin{figure*}[htbp!]
\centering
\includegraphics[width=\textwidth]{img/sample-questions.pdf}
\caption{Two sample sentence completion questions with the three primary components labeled: a passage \( \mathit{P} \), a series of discrete blanks \( \mathit{B} \), and a set of answer choices \( \mathit{C} \) for each blank (Section \ref{sec:data}). Both questions were scraped from public websites and examination sources (The Princeton Review, 2011).}
\label{fig:sampleqs}
\end{figure*}

Given that the intent to evaluate pretrained language models, there data was not split into training, development, and evaluation sets following standard guidelines from previous work with similar datasets \cite{woods-2016-exploiting, huang-lifu-2019-cosmosQA}. This paper reports high variability in the average number of blanks per passage for the dataset constructed, though most blanks correspond to a set of three answer choices. 

\subsection{Text Completion Methods}
\label{sec:methods}

In order to complete the sentence completion tasks, various pre-trained language models were used. With a formal definition, let \( \mathit{C} = {c_1, c_2, ..., c_n} \) be the answer choices corresponding to a given question \( \mathit{Q} \) in the dataset. Then, the language modeling task can be understood as selecting the option that maximizes the joint probability \( P(c_i | Q\)); in other words, the answer choice with the highest probability of being associated with its context, given the passage \( \mathit{P} \) and the corresponding blank.

As such, following \citet{devlin-jacob-2019-BERT}, we apply the same tokenizer to derive the sequence: [[CLS], \( \mathit{P} \), [SEP], \( \mathit{B} \), [SEP], \( \mathit{C} \)]; both [CLS] and [SEP] are tokens used in transformer-based models, where the former specifies the beginning of an input sentence (that will be eventually represented as a vector) and the latter denotes the end of that sentence. Note that this approach is generalizable and can take any transformer as the encoder, though the paper presents pre-trained BERT as the method used \cite{devlin-jacob-2019-BERT}. To improve on the BERT large uncased model\footnote{https://github.com/huggingface/transformers}, our approach involves fine-tuning by treating all questions with the correct answer choices labeled as 1, while all questions with incorrect answer choices are labeled as 0. For example, in reference to Figure \ref{fig:sampleqs}, the second passage would have "dogmatic" and "checking" as the correct answers to the first and second blanks respectively; all other answer choice combinations would have been deemed as incorrect (thus labeled as 0) and fed into the language modeling neural networks as incorrect examples. Then, we follow the same protocol as previously described for BERT \cite{devlin-jacob-2019-BERT} using this classification scheme to fine-tune the pre-trained BERT model; the contextual vectors are used as opposed to the solely the [CLS] token.

Furthermore, we compare this approach with several baseline methods to allow for comparative analyses in terms of model accuracy (defined as the number of questions with correct answer choices for all blanks); the state-of-the-art methods chosen are all pre-trained language models used to establish baseline performance in other similar works focused on evaluating text completion and reading comprehension datasets \cite{woods-2016-exploiting, berzak-yevgeni-2020-STARC}. These unsupervised models leverage pre-training on a large corpus of English texts to learn representations of the language and ultimately support downstream tasks like our sentence completion challenge:
\begin{itemize}
    \item \textbf{BERT} \cite{devlin-jacob-2019-BERT}. A pre-trained bidirectional transformer language model that learns contextual representations; as described above, a sequence of [[CLS], \( \mathit{P} \), [SEP], \( \mathit{B} \), [SEP], \( \mathit{C} \)] for each question is tokenized according to standard protocol described by \citet{devlin-jacob-2019-BERT}, converted into word embeddings and vectors, and processed through all encoder layers to produce the hidden states requried to select the answer choice with maximal probability of \( P(c_i | Q\)).
    \item \textbf{RoBERTa} \cite{liu-etal-2019-roberta}. Improved version of BERT that features dynamic masking (such that the masking pattern changes with each sequence) and larger batch-training sizess; the same protocols for BERT are utilized here.
\end{itemize}
Finally, with both the advanced, fine-tuned approach and baseline models, we compute accuracy scores as defined by the number of questions with correct answer choices across all blanks from the dataset; this is done by comparing the predicted answers from the transformer language models to the actual answers included for each question (refer to Section \ref{sec:data} for details).

==> tex_old/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We introduce a novel dataset that incorporates common text completion and sentence equivalence questions from standardized examinations, allowing us to evaluate the performance of popular off-the-shelf language modeling architecture. We leverage this to present empirical results comparing state-of-the-art neural architectures, and demonstrate that the RoBERTa models perform significantly better than the BERT models. Our experiments further reveal that performance generally decreases with questions rated as higher difficulty by official examination sources (such as the Educational Testing Service for GRE questions), agnostic of the type of model used. Our results demonstrate inherent differences in text completion capabilities for pretrained language models, and extend integration of contextual information and relational answers as exciting directions for future work. The significant gap between human and machine performance on standardized examination questions reveals substantial room for improvement in model performance, and we plan to tackle this by engineering more sophisticated attention mechanisms to focus on the areas of a given question where the most relevant information is located. In addition, the decrease in model performance across 2- and 3-blank questions encourages future research on optimizing overall accuracy when there are multiple slots in a language modeling task.

==> tex_old/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

INSTRUCTIONS (DELETE LATER) 
Experiments/Results (experiments)
    Data description
    Exploratory data analysis, preprocessing, feature extraction, feature selection: Enough to ensure your experiments can be replicated by others
    Modeling choices: What models did you select? Why? How were parameters determined? Other design choices such as subsampling, oversampling, etc.
    Empirical results and comparisons (figures and tables)


    
\subsection{Data Exploration}
As stated in the introduction, our data comes from students interacting with the \textit{Jo Wilder and the Capitol Caese} game. The data consists of 23.6 million user interactions which includes clicking on multiple types of objects, hovering over maps or objects, and reaching checkpoints. Each observation comes from one of 23.5 thousand user sessions. Each session is split into 23 levels (0 to 22). At the end of each level, there is a question. Data from the first 18 questions were provided in a separate data set. We have 424 thousand observations. Almost 300 thousand of the questions were answered correctly, and the other 124 thousand were answered incorrectly. 
DESCRIBE THE FEATURES

\subsection{Pre-Processing}
As we had many more observations than we did labels, we needed to aggregate the data for each level. We tried many methods in order to find the best method for each feature. For numerical features, we used mean, sum, min, and max for aggregation. For categorical features, we used count and nunique. 
We use Pearson correlation coefficients in order to choose which features to include in our data. We selected the aggregation method that correlated the most with our label (whether the student answered the question correctly or not) and made sure that none of the features that we kept were correlated with each other. Additionally, we used importance as another method of checking which of our variables we should keep.

WHICH FEATURES DID WE USE???????

We split our data 80-20 in order to have a training and a testing set.

\includegraphics[scale = 0.4]{imporance.png}











DELETE BELOW:
This section presents a series of experiments to assess off-the-shelf language modeling architecture on verbal reasoning questions from standardized examinations, with questions sourced from official and unofficial Graduate Record Examinations (GRE) practice tests as described in Section \ref{sec:approach}. In addition, this paper further demonstrates direct benchmark comparisons between human and machine performance to evaluate question quality in the novel dataset.

\subsection{Language Modeling Evaluation}
\label{sec:lmresults}

To assess machine performance on verbal reasoning questions, sample GRE questions from the novel dataset produced in this paper were utilized (refer to Section \ref{sec:approach} for details on the sources and statistics of questions), given the lack of available annotated datasets that accurately reflect standardized examination text completion- and sentence equivalence-style formats (as opposed to large-scale reading comprehension datasets such as RACE by \citet{lai-guokun-2016-RACE}). In addition, all of our models are also evaluated on the Microsoft Research Sentence Completion Challenge \cite{zweig-burges-2012-challenge} to compare model performance against benchmark scores from prior work and validate the generalizability of our approach. As described previously, since the primary objective is to evaluate performance of off-the-shelf language modeling architecture, the models used here do not involve any additional training other than the standard pre-training that is already implemented \cite{devlin-jacob-2019-BERT, liu-etal-2019-roberta}; as such, no data split for training, development, evaluation, or cross-validation is presented here since every entry in the dataset is used for evaluation. 

To further augment the pool of sample questions and increase generalizability to a range of sentece completion problems (in terms of difficulty, format, and word choice), questions that involved multiple blanks were also scraped and processed into multiple standard "one-blank" questions (Figure \ref{fig:processing}). As such, a total of 305 questions were evaluated by each of the models, with a breakdown of 162, 98, and 45 questions labeled as extracted from 1-blank, 2-blank, and 3-blank questions respectively (refer to Table \ref{tab:experimentresults}).

\begin{figure}[htbp!]
\centering
\includegraphics[width=\columnwidth]{img/Sample3Slot.pdf}
\caption{Example of how a sample sentence completion question with three blanks is processed into three single-blank sentence completion questions; only one blank is left within each processed question, with the other two blanks filled with the correct answer (colored blue). This question was scraped from an official examination source (Educational Testing Service, 2017).}
\label{fig:processing}
\end{figure}

In this experiment, we benchmark two primary state-of-the-art language models following extensive prior work in this area \cite{gardner-matt-2019-RCmorecomprehensive, huang-lifu-2019-cosmosQA, berzak-yevgeni-2020-STARC} as follows:
\begin{itemize}
    \item \textbf{BERT} \cite{devlin-jacob-2019-BERT}. A bidirectional transformer language model that learns contextual representations and is already pretrained on a large corpus of English data for masked language modeling, as originally described by \citet{devlin-jacob-2019-BERT}; here, it is adapted as our baseline model and both the base and large architectures (cased) are utilized in order to compare performance on verbal reasoning questions and assess whether an increased number of encoder layers results in higher accuracy.
    \item \textbf{RoBERTa} \cite{liu-etal-2019-roberta}. Improved version of BERT that features dynamic masking (such that the masking pattern changes with each sequence) and increased pretraining with more epochs and larger batch sizes (with the same masked language modeling objective described for BERT); here, it is adapted as our advanced model, with three separate versions used to gauge comparative performance: DistilRoBERTa (distilled version with only 6 layers and is twice as fast as the original RoBERTa base model), RoBERTa base, and RoBERTa large. In particular, they are included with the objective of assessing the tradeoff between speed (due to model complexity) and accuracy, in addition to performance increases compared to BERT.
\end{itemize}

As described previously, since the aim of this paper is to evalulate off-the-shelf language modeling architecture, no additional training was performed and thus no specific experimental settings (number of epochs, learning rate, training efficiency, batch size, etc.) and model development specifics can be reported. However, it is important to note that accuracy is defined as the number of sample questions that the language model correctly identifies the correct answer for (by indicating a candidate with the highest probability above all others) divided by the number of total questions in the dataset, which is the core metric used to evaluate model performance in these experiments; this follows previous work done by \citet{zweig-burges-2012-challenge} and \citet{berzak-yevgeni-2020-STARC}.

Table \ref{tab:experimentresults} provides a comparison of accuracy values for each of the models tested\footnote{Note that JP Selame ran the DistilRoBERTa, RoBERTa Base, and RoBERTa Large models for all question types, while Anthony Wang ran the BERT Base and BERT Large models for all question types; we shared our accuracy results in order to complete this section individually.}, in addition to a human evaluator, demonstrating that the RoBERTa models (DistilRoBERTa, RoBERTa Base, RoBERTa Large) perform significantly better than the BERT models (BERT Base, BERT Large) across all three question types (1-, 2-, 3-blanks).

\begin{table}[htbp!]
\centering\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cccc} 
\toprule
\bf Language Model & \bf 1-blank & \bf 2-blank & \bf 3-blank & \bf Overall \\
\midrule
BERT Base & 46.30 & 29.59 & 20.00 & 37.70 \\
BERT Large & 47.53 & 26.53 & 17.78 & 35.74 \\
DistilRoBERTa & 51.23 & 32.65 & 24.44 & 41.31 \\
RoBERTa Base & 58.64 & 38.78 & 28.88 & 47.87 \\
RoBERTa Large & 62.96 & 42.86 & 33.33 & 52.13 \\
\hline
Humans & 81.88 & 77.27 & 71.43 & 80.89 \\
\bottomrule
\end{tabular}}
\caption{Performance accuracy on GRE question dataset, with random baseline as 20.00, 10.89, 3.59 for 1-blank, 2-, and 3-blank questions respectively (there are 5 candidates as answer choices for each 1-blank question, whereas only 3 candidates for that of 2- or 3-blank questions). All models are off-the-shelf and have not been finetuned or further trained beyond the pretraining detailed in the original work \cite{devlin-jacob-2019-BERT, liu-etal-2019-roberta}.}
\label{tab:experimentresults}
\end{table}

It is notable that for the RoBERTa models, increased complexity with a higher number of encoder layers is strongly correlated with an increase in accuracy performance with the GRE questions (for all three question types, 1-blank, 2-blank, and 3-blank), which has been demonstrated in prior work \cite{zweig-burges-2012-challenge, berzak-yevgeni-2020-STARC}; this is likely due to better optimization of pretraining with dynamic masking, larger batch sizes, and more epochs compared to BERT, especially given that GRE questions are specifically designed to tease out nuances in sentence structure and overall passage meaning. The results for RoBERTa Large peak at an accuracy of 33.33\% for 3-blank questions, nearly doubling that of BERT large, though the fact that the random baseline also changes must be taken into account as a confounding factor. It is interesting, however, that the BERT accuracy results for the large model are actually lower than those of the base model for 2- and 3-blank questions (57.14, 53.33 vs. 50.00, 46.67 respectively); this is likely due to a relatively lower number of sample questions (98, 45 respectively), which could reflect poor diversity in terms of difficulty, passage length, and word choice, thus confounding the results (a more thorough analysis can be found in Section \ref{sec:analysis}). Notably, maximum performance scores derived from our experiments are similar to those of prior work, albeit with different datasets that are more focused on reading comprehension and summarization; RoBERTa Large performance on two state-of-the-art datasets that mirror standardized examinations, RACE and OneStopQA \cite{berzak-yevgeni-2020-STARC}, was 82.29 and 85.60 respectively. On the other hand, the maximum performance scores with RoBERTa Large in our experiments improves upon that of older dependancy and n-gram models such as pointwise mutual information (Table \ref{tab:microsoft}), which had an accuracy of 61.44 based on the Microsoft Research Sentence Completion Challenge dataset \cite{zweig-burges-2012-challenge}.

\begin{table}[htbp!]
\centering\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c} 
\toprule
\bf Language Model & \bf \% accuracy \\
\midrule
N-gram \cite{zweig-burges-2012-challenge} & 39.00 \\
Labeled Dependancy \cite{gubbins-vlachos-2013-dependency} & 48.30 \\
LSA \cite{zweig-burges-2012-challenge} & 49.00 \\
BERT Base & 55.96 \\
BERT Large & 59.71 \\
PMI \cite{zweig-burges-2012-challenge} & 61.44 \\
DistilRoBERTa & 64.81 \\
RoBERTa Base & 70.37 \\
RoBERTa Large & 74.07 \\
\hline
Humans & 91.00 \\
\bottomrule
\end{tabular}}
\caption{Performance accuracy on MSR Sentence Completion Challenge dataset. All models are off-the-shelf and have not been finetuned or further trained beyond the pretraining detailed in the original work \cite{devlin-jacob-2019-BERT, liu-etal-2019-roberta}.}
\label{tab:microsoft}
\end{table}

Lastly, human performance is consistently higher across all question types and is approximately 17\% higher for the overall weighted accuracy; of particular interest is the result for 3-blank questions, where human performance is nearly matched by machine performance with the RoBERTa Large model (again, it is likely confounded by the relatively smaller sample size of questions, however). It is plausible that current state-of-the-art language models are closing the gap for performance improvements compared to humans on sentence completion questions, especially with relatively complex transformers that have been thoroughly optimized. These human accuracy results can additionally serve as a performance ceiling for comparison with other models in the future.



==> tex_old/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

A radical shift that is currently transforming the field of education is the adoption of technology to facilitate student learning and growth in school; widespread usage of tablets, laptops, and mobile devices in primary and secondary education enables a universe of possibilities in terms of leveraging digital technology to enhance student learning \cite{schindler-2023-engagement}.  

In particular, game-based learning is an educational intervention that has received extensive interest in the field of pedagogy, for three key reasons. First, it has been proposed to increase student engagement, given that the elements of discovery, immersion, and feedback inherent to game-based environments can pique students' curiosity and motivate them to master the accompanying educational material. Existing evidence demonstrates that students in primary and secondary school exhibit lower learning anxiety when playing educational games instead of listening to traditional lectures, in addition to an increase in both motivation and academic performance within the context of several STEM disciplines \cite{hung-2014-digitallearning, ciloglu-2023-ARbiology}. Second, a key advantage of game-based learning and digital approaches in general is the increased accessibility and scale; akin to online platforms like Coursera and Udemy, these interventions could address educational inequalities and widen access to millions of students globally, particularly those in low-income homes or developing countries \cite{haleem-2022-digital}. Lastly, game-based learning offers the possibility of personalized approaches, such that the games are tailored and adapted to the skill level of each student. Thus, in spite of the fundamentally challenging and time-consuming task of developing educational games that are in alignment with current pedagogical guidelines and that cover different academic disciplines, work in the domain of game-based learning is crucial given its ability to promote student outcomes and skill development.

However, for game-based learning approaches to be effective, the underlying engine must accurately predict a student's performance throughout the game; otherwise,  feedback (e.g., hints, suggestions) and in-game checkpoints will not be implemented appropriately, such that students remain engaged with the material and are continually improving as they learn from the game. Despite significant advances in the development of several game-based frameworks \cite{min-2017-multimodal} and theoretical student learning models \cite{mayer-2019-games}, research on knowledge tracing has lagged behind, primarily due to the lack of large-scale, open-source datasets from game-based learning platforms that have amassed a significant population of student users. Furthermore, though knowledge tracing and characterization of a student's mastery level have been investigated in intelligent tutoring systems \cite{haridas-KT}, there has been little work focused on evaluating what specific features of a game-based learning environment support effective learning experiences for student; this is crucial given its implications in question design and pedagogical guidelines, in addition to the idea that we can only iterate and improve on these game-based approaches if we know what parts of the gameplay experience are driving the most and least learning.

In order to address the paucity of available evidence in these areas, we leverage student gameplay data from \textit{Jo Wilder and the Capitol Caese}, a popular educational game designed for students in elementary school and focused on the skills of historical analysis and reading comprehension; the dataset was released to encourage efforts to improve predictive student modeling and knowledge tracing (discussed above), which will ultimately help improve the gameplay design and enhance learning outcomes \cite{wardrip2022jo}. We hypothesize that by leveraging one of the only existing compiled databases of student gameplay interactions in a historical inquiry game, we can better determine the features that are most predictive of student performance and correct question answering. In addition, our empirical findings establish complete benchmarks in terms of several machine learning models, which will be discussed in Section \ref{sec:approach}. In summary, this paper makes four main contributions as follows:
\begin{enumerate}
    \item We leverage an open-access dataset \textbf{
    \item Fill in
    \item Fill in
\end{enumerate}

This work will facilitate the further development of game-based learning approaches, especially in the context of question and gameplay design; to the best of our knowledge, this is the first work to [Fill in].

==> tex_old/related-work.tex <==
\section{Background and Related Work}
\label{sec:related-work}


Recent work on evaluating game-based learning approaches has spanned a variety of domains in STEM and the humanities, including but not limited to biology, mathematics, and reading comprehension \cite{hung-2014-digitallearning, min-2017-multimodal, ciloglu-2023-ARbiology}. However, most of the existing research has taken the perspective of investigational studies, focused on interviewing students and understanding factors such as their motivation, engagement, and performance while playing different educational games; this is in contrast to directly modeling student knowledge (i.e., knowledge tracing) and leveraging computational approaches to determine how much a student has mastered the material.

\citet{chu-concept-mathematics} improved on these qualitative approaches by introducing quantitative metrics to represent a student's comprehension for different mathematical concepts in a primary school educational game, including competencies such as the multiplication of integers and fractions. By scoring each question in the game with a relevancy index (i.e., to explictly label what learning objective each question was designed to address), the in-game checkpoint assessment scores were used to decide which of three alternative learning paths was presented to the students; thus, this allowed the underlying game engine to adopt a diagnostic approach, such that students who have not yet attained the expected learning outcomes are instructed with further supplementary content. The post-gameplay scores demonstrated that students on average scored approximately 13\% higher than students who listened to traditional lecture \cite{chu-concept-mathematics}. Despite these advances, however, it is evident that multiple layers of information were left out from consideration, including but not limited to how much time was spent in each game session, what text the students saw, which questions they spent the most time on, where they placed their cursor, and what coordinates in the game they clicked on.

In particular, \citet{geden_emerson_carpenter_rowe_azevedo_lester_2020} utilized similar time-stamped gampelay features (in-game assessment scores, level of the game that a student is on, what the students are clicking and which gameplay actions they engage in) to predict student microbiology content knowledge, achieving the optimal F1-score of 0.65 with a linear support vector machine (SVM) and 0.63 with k-nearest neighbors (KNN). These features are similar to those that are available to us with the \textit{Jo Wilder} dataset, which will be further explored in Section \ref{sec:approach}; however, since this dataset is novel, we are unable to disclose any comparative metrics. To the best of our knowledge, machine learning approaches to model student mastery has not been performed on a historical inquiry game of this scale.

Furthermore, it is important to note that several pioneering studies have begun to incorporate multimodal data to augment model performance in terms of knowledge tracing; \citet{emerson-multimodal} took advantage of not only student gameplay interactions, but also data on facial expression and eye gaze captured by camera sensors on the computer workstations students were using. Applying a logistic regression model, a F1-score of 0.607 was achieved, demonstrating that complex multimodal, data inputs may not necessarily translate to better knowledge tracing as compared to previous work by \citet{geden_emerson_carpenter_rowe_azevedo_lester_2020}. As such, in the context of this study, we decide to make use of only gameplay interactions, and address gaps in the literature by examining whether certain features from student in-game interaction data from a historical inquiry game disproportionately account for accurate predictions on whether a student correctly answers an in-game assessment question or not (i.e., as a proxy for student mastery of the material). Our work is distinguished because we propose to evaluate [fill in].


